Planck intermediate results. XXXIX. The Planck list of high-redshift source candidates

The Planck mission, thanks to its large frequency range and all-sky coverage, has a unique potential for systematically detecting the brightest, and rarest, submillimetre sources on the sky, including distant objects in the high-redshift Universe traced by their dust emission. A novel method, based on a component-separation procedure using a combination of Planck and IRAS data, has been applied to select the most luminous cold submm sources with spectral energy distributions peaking between 353 and 857GHz at 5' resolution. A total of 2151 Planck high-z source candidates (the PHZ) have been detected in the cleanest 26% of the sky, with flux density at 545GHz above 500mJy. Embedded in the cosmic infrared background close to the confusion limit, these high-z candidates exhibit colder colours than their surroundings, consistent with redshifts z>2, assuming a dust temperature of 35K and a spectral index of 1.5. First follow-up observations obtained from optical to submm have confirmed that this list consists of two distinct populations. A small fraction (around 3%) of the sources have been identified as strongly gravitationally lensed star-forming galaxies, which are amongst the brightest submm lensed objects (with flux density at 545GHz ranging from 350mJy up to 1Jy) at redshift 2 to 4. However, the vast majority of the PHZ sources appear as overdensities of dusty star-forming galaxies, having colours consistent with z>2, and may be considered as proto-cluster candidates. The PHZ provides an original sample, complementary to the Planck Sunyaev-Zeldovich Catalogue; by extending the population of the virialized massive galaxy clusters to a population of sources at z>1.5, the PHZ may contain the progenitors of today's clusters. Hence the PHZ opens a new window on the study of the early ages of structure formation, and the understanding of the intensively star-forming phase at high-z.

==> PlanckTable.tex <==
%Planck table template file, to be used with A&A style and Planck.tex to produce Planck tables %  for publication.
%
% version 11 September 2011 ---  CRL

\begin{table*}[tmb]                 % table* is a two-column table.  Drop the * for one column.
\begingroup
\newdimen\tblskip \tblskip=5pt
\caption{}                          % Caption goes here.
\label{}                            % Label goes here.
\nointerlineskip
\vskip -3mm
\footnotesize
\setbox\tablebox=\vbox{
   \newdimen\digitwidth 
   \setbox0=\hbox{\rm 0} 
   \digitwidth=\wd0 
   \catcode`*=\active 
   \def*{\kern\digitwidth}
%
   \newdimen\signwidth 
   \setbox0=\hbox{+} 
   \signwidth=\wd0 
   \catcode`!=\active 
   \def!{\kern\signwidth}
%
\halign{                            % Template goes here.
\noalign{\doubleline}
                                    % Table headings go here.
\noalign{\vskip 3pt\hrule\vskip 5pt}
                                    % Body of table goes here.
\noalign{\vskip 5pt\hrule\vskip 3pt}}}
%\endPlancktable                    % ends one-column \halign
\endPlancktablewide                 % ends two-column \halign
\tablenote a Footnote a.\par
\tablenote b Footnote b.\par
\endgroup
\end{table*}                        % table* is a two-column table.  Drop the * for one column.

